Architectural Analysis of FPGA Technology Impact

The use of high-level languages for designing hardware is gaining popularity since they increase design productivity by providing higher abstractions. However, one drawback of such abstraction level has been the difficulty of relating the low-level implementation problems back to the original high-level design, which is paramount for architectural optimization. In this work (developed between April 2013 and April 2014), we propose a methodology to analyze the effects of technology over the architecture, and to generate architectural-level area, delay and power metrics. Such feedback allows the designer to quickly gauge the impact of architectural decisions on the quality of generated hardware and opens the door to automatic architectural analysis. We demonstrate the use of our technique on three FPGA platforms using two designs: a Reed-Solomon error correction decoder and a 32-bit pipelined processor implementation.

==> maps.tex <==

\begin{figure*}[t!]
  \centering
  \subfloat[Spartan 6 area map. \label{fg:smips_map_a_s6}]{
    \includegraphics[width=0.185\textwidth]{Graphics/smips_map_a_s6.pdf}
  }
  \subfloat[Virtex 5 area map. \label{fg:smips_map_a_v5}]{
    \includegraphics[width=0.185\textwidth]{Graphics/smips_map_a_v5.pdf}
  }
  \subfloat[Virtex 7 area map. \label{fg:smips_map_a_v7}]{
    \includegraphics[width=0.185\textwidth]{Graphics/smips_map_a_v7.pdf}
  }
  \subfloat[Spartan 6 delay map. \label{fg:smips_map_d_s6}]{
    \includegraphics[width=0.185\textwidth]{Graphics/smips_map_d_s6.pdf}
  }
  \subfloat[Virtex 5 delay map. \label{fg:smips_map_d_v5}]{
    \includegraphics[width=0.185\textwidth]{Graphics/smips_map_d_v5.pdf}
  }
  \\
  \subfloat[Virtex 7 delay map. \label{fg:smips_map_d_v7}]{
    \includegraphics[width=0.185\textwidth]{Graphics/smips_map_d_v7.pdf}
  }
  \subfloat[Spartan 6 power map. \label{fg:smips_map_p_s6}]{
    \includegraphics[width=0.185\textwidth]{Graphics/smips_map_p_s6.pdf}
  }
  \subfloat[Virtex 5 power map. \label{fg:smips_map_p_v5}]{
    \includegraphics[width=0.185\textwidth]{Graphics/smips_map_p_v5.pdf}
  }
  \subfloat[Virtex 7 power map. \label{fg:smips_map_p_v7}]{
    \includegraphics[width=0.185\textwidth]{Graphics/smips_map_p_v7.pdf}
  }
  \subfloat{
    \includegraphics[width=0.185\textwidth]{Graphics/smips_map_legend.pdf}
  }
  \caption{SMIPS area, delay and power heat maps for Spartan 6, Virtex 5 and Virtex 7.}\label{fg:smips_maps}
\end{figure*}



==> testcases.tex <==
\subsection{Test cases}
\label{sec:testcases}
%\textcolor{red}{Describe test-cases, different sizes of examples -- why this choice}

%\textcolor{red}{Description of each design and sub-modules}

We have chosen two high-level hardware designs as test cases, with distinct properties in terms of performance, complexity, size, behavior, etc. Both test cases have aggressive performance requirements and resource constraints. Each is specified as a hierarchical design with a significant number of modules, sub-modules and rules. 
%{SKIP}In this section we describe the test cases and their architecture.

%\textbf{GCD:} A simple hardware implementation of the Greatest Common Divisor calculator. It implements the classical Euclid's algorithm with 32-bit natural numbers. This architecture is very small and only requires two rules --subtract and swap.

\textbf{Reed-Solomon:} This design implements a parameterized Reed-Solomon error correction decoder. 
%{SKIP}The decoder can be configured by user determined values of the size of the input data block and the number of parity characters, which determine the maximum number of correctable errors. 
At 100 MHz, it meets the throughput requirement for use in an 802.16 wirelesses receiver. Reed-Solomon decoding algorithm is composed of several steps, each of which is implemented as a separate module shown in Figure~\ref{fg:rs_arch}. To quantify the dynamic activity used for generating the power score metrics of the decoder design, we chose a realistic testbench that generates input data with errors at 50\% of the maximal correctable rate.

\begin{figure}[ht]
 \small\centering
  \includegraphics[width=\columnwidth]{Graphics/rs_arch.pdf}
 \caption{\label{fg:rs_arch} Reed-Solomon decoder}
\end{figure}


\textbf{SMIPS:} This design comprises of a 32-bit RISC microarchitecture that implements the MIPS I ISA. It includes a multiply unit, coprocessor 0, where MIPS I implements the data and instruction TLBs, independent instruction/data L1 caches, and a unified, N-way L2 cache. This 5-stage processor can boot the GNU/Linux kernel and it is targeted to run at 100 MHz. Dynamic activity generated during booting of Linux is used to generate the power score metrics of the SMIPS design.

\begin{figure}[thb]
 \centering
 \includegraphics[width=0.6\columnwidth]{Graphics/smips_arch.pdf}
 \caption{SMIPS RISC architecture.}
 \label{fg:smips_arch}
\end{figure}

In Figure~\ref{fg:smips_arch} the main architectural elements of SMIPS are shown. Some blocks are encapsulated in a single rule --e.g. the pipeline stages-- while others are implemented in modules. Some blocks contain contain or instantiate other elements. The partition and distribution of architectural elements in rules or modules responds to both architectural or source code organization reasons. For simplicity, only the main connections between elements are shown --for instance, the control path of the pipeline is not shown.


